Controllers with Minimal Observation Power (Application to Timed Systems)

We consider the problem of controller synthesis under imperfect information in a setting where there is a set of available observable predicates equipped with a cost function. The problem that we address is the computation of a subset of predicates sufficient for control and whose cost is minimal. Our solution avoids a full exploration of all possible subsets of predicates and reuses some information between different iterations. We apply our approach to timed systems. We have developed a tool prototype and analyze the performance of our optimization algorithm on two case studies.

==> implementation.tex <==
\section{Implementation}\label{implementation}

The original algorithm for solution of a partial observability timed game with a \emph{fixed} set of observable predicates \cite{cdllr07} has been implemented in the {\sc Uppaal-Tiga} tool.
One can use {\sc Uppaal-Tiga} as a blackbox in the implementation of our lattice-based algorithm.
However, in this case it would not possible to take advantage of one of the contributions of our method: reusage of the information between game solutions for different observation sets.

Thus we reimplemented the whole algorithm as a prototype written in the Python language.
The implementation uses our Python framework for Timed Automata manipulation\footnote{\url{http://cs.aau.dk/~peterbul/python.html}} and uses the {\sc Uppaal DBM} library and the  Timed Automata models parser.
